Probabilistic Constraint for Safety-Critical Reinforcement Learning

In this paper, we consider the problem of learning safe policies for probabilistic-constrained reinforcement learning (RL). Specifically, a safe policy or controller is one that, with high probability, maintains the trajectory of the agent in a given safe set. We establish a connection between this probabilistic-constrained setting and the cumulative-constrained formulation that is frequently explored in the existing literature. We provide theoretical bounds elucidating that the probabilistic-constrained setting offers a better trade-off in terms of optimality and safety (constraint satisfaction). The challenge encountered when dealing with the probabilistic constraints, as explored in this work, arises from the absence of explicit expressions for their gradients. Our prior work provides such an explicit gradient expression for probabilistic constraints which we term Safe Policy Gradient-REINFORCE (SPG-REINFORCE). In this work, we provide an improved gradient SPG-Actor-Critic that leads to a lower variance than SPG-REINFORCE, which is substantiated by our theoretical results. A noteworthy aspect of both SPGs is their inherent algorithm independence, rendering them versatile for application across a range of policy-based algorithms. Furthermore, we propose a Safe Primal-Dual algorithm that can leverage both SPGs to learn safe policies. It is subsequently followed by theoretical analyses that encompass the convergence of the algorithm, as well as the near-optimality and feasibility on average. In addition, we test the proposed approaches by a series of empirical experiments. These experiments aim to examine and analyze the inherent trade-offs between the optimality and safety, and serve to substantiate the efficacy of two SPGs, as well as our theoretical contributions.

==> fig_dualVariables_Safe.tex <==
%!TEX root = root.tex
\begin{tikzpicture}
	\pgfplotsset{grid style={dashed,gray!50}}
	\begin{axis}[
		tick scale binop=\times,
		%title style={yshift=-1ex},
		%xlabel near ticks,
		%ylabel near ticks,
		minor y tick num=0,
		minor x tick num=1,
		ytick={0,5,...,25},		
		%title={},
		xlabel={Iteration ($k$)},
		ylabel={Dual Variable},
		ylabel near ticks,
		width=\columnwidth, 
		height=0.45\columnwidth, 
		xmin=0,xmax=10000,ymin=0,ymax=25,
		grid=both,
		legend style={
			at={(0.98,0.06)}, 
			anchor=south east, 
			legend cell align=left
			}
	]
	\addplot [color=red,solid,thick,mark=none,mark options={red,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataDualVariableSafe.dat};
	\addlegendentry{Dual Variable $\lambda$};
	
\end{axis}
\end{tikzpicture}

==> fig_map_NoSafe.tex <==
%!TEX root = root.tex
\begin{tikzpicture}
	\pgfplotsset{grid style={dashed,gray!50}}
	\begin{axis}[
		minor tick num=1,
		%xtick={1,3,...,15},	
		%ytick={1,3,...,15},
		xtick={0.5,2.5,...,14.5},
		xticklabels ={1,3,...,15},
		ytick={0.5,2.5,...,14.5},
		yticklabels ={1,3,...,15},
		extra x ticks={1,3,...,15},			
		extra x tick labels={},        	
		extra y ticks={1,3,...,15},			
		extra y tick labels={},     
        extra tick style={
            grid=both,
        },					
		%title={},
		width=0.8\columnwidth, 
		height=0.8\columnwidth, 
		xmin=0,xmax=15,ymin=0,ymax=15,
		%grid=both,
		legend columns=3,
		legend style={
			font=\scriptsize,
			at={(0.94,0.98)}, 
			anchor=north east, 
			legend cell align=left
			}
	]
	\draw [draw=black,fill=black] (0,0) rectangle (10,150);
	\draw [draw=black,fill=black] (0,0) rectangle (150,10);
	\draw [draw=black,fill=black] (140,0) rectangle (150,150);
	\draw [draw=black,fill=black] (0,140) rectangle (150,150);
	
	\draw [draw=black,fill=black] (60,0) rectangle (90,70);
	\draw [draw=black,fill=black] (60,150) rectangle (90,80);

	\draw [draw=gray,fill=gray!50] (30,120) rectangle (40,130);
	\draw [draw=gray,fill=gray!50] (100,20) rectangle (110,30);

	\addplot [color=red,solid,thick,mark=*,mark options={red,solid}]
		table[x index=2,y index=1, col sep=comma]{figures/data/dataTrajectoryNoSafeLambda0.dat};
	\addlegendentry{$\lambda=0$};

	\addplot [color=green,solid,thick,mark=*,mark options={green,solid}]
		table[x index=2,y index=1, col sep=comma]{figures/data/dataTrajectoryNoSafeLambda30.dat};
	\addlegendentry{$\lambda=30$};			
		
	\addplot [color=blue,solid,thick,mark=*,mark options={blue,solid}]
		table[x index=2,y index=1, col sep=comma]{figures/data/dataTrajectoryNoSafeLambda60.dat};			
	\addlegendentry{$\lambda=60$};
		

\end{axis}
\end{tikzpicture}


==> fig_map_Safe.tex <==
%!TEX root = root.tex
\begin{tikzpicture}
	\pgfplotsset{grid style={dashed,gray!50}}
	\begin{axis}[
		minor tick num=1,
		%xtick={1,3,...,15},	
		%ytick={1,3,...,15},
		xtick={0.5,2.5,...,14.5},
		xticklabels ={1,3,...,15},
		ytick={0.5,2.5,...,14.5},
		yticklabels ={1,3,...,15},
		extra x ticks={1,3,...,15},			
		extra x tick labels={},        	
		extra y ticks={1,3,...,15},			
		extra y tick labels={},     
        extra tick style={
            grid=both,
        },
		width=0.8\columnwidth, 
		height=0.8\columnwidth, 
		xmin=0,xmax=15,ymin=0,ymax=15,
		%grid=both,
		legend style={
			at={(0.98,0.22)}, 
			anchor=south east, 
			legend cell align=left
			}
	]
	\draw [draw=black,fill=black] (0,0) rectangle (10,150);
	\draw [draw=black,fill=black] (0,0) rectangle (150,10);
	\draw [draw=black,fill=black] (140,0) rectangle (150,150);
	\draw [draw=black,fill=black] (0,140) rectangle (150,150);
	
	\draw [draw=black,fill=black] (60,0) rectangle (90,70);
	\draw [draw=black,fill=black] (60,150) rectangle (90,80);

	\draw [draw=gray,fill=gray!50] (30,120) rectangle (40,130);
	\draw [draw=gray,fill=gray!50] (100,20) rectangle (110,30);

	\addplot [color=red,solid,thick,mark=*,mark options={red,solid}]
		table[x index=2,y index=1, col sep=comma]{figures/data/dataTrajectorySafe.dat};

\end{axis}
\end{tikzpicture}


==> fig_probabilities_NoSafe.tex <==
%!TEX root = root.tex
%\begin{tikzpicture}
%	\pgfplotsset{grid style={dashed,gray!50}}
%	\begin{axis}[
%		%title style={yshift=-1ex},
%		%xlabel near ticks,
%		%ylabel near ticks,
%		minor tick num=1,
%		%title={},
%		xlabel={Time ($t$)},
%		ylabel={Probability},
%		ylabel near ticks,
%		width=\columnwidth, 
%		height=0.75\columnwidth, 
%		xmin=0,xmax=10000,ymin=0,ymax=1,
%		grid=both,
%		legend style={
%			at={(0.98,0.22)}, 
%			anchor=south east, 
%			legend cell align=left
%			}
%	]
%	\addplot [color=red,solid,thick,mark=none,mark options={red,solid}]
%		table[x index=0,y index=1, col sep=comma]{figures/data/dataProbabilitySafetyNoSafeLambda0.dat};
%	\addlegendentry{$\lambda=0$ - Safety};
%	\addplot [color=red,dashed,thick,mark=none,mark options={red,solid}]
%		table[x index=0,y index=1, col sep=comma]{figures/data/dataProbabilityGoalNoSafeLambda0.dat};
%	\addlegendentry{$\lambda=0$ - Goal};
%
%	\addplot [color=green,solid,thick,mark=none,mark options={green,solid}]
%		table[x index=0,y index=1, col sep=comma]{figures/data/dataProbabilitySafetyNoSafeLambda30.dat};
%	\addlegendentry{$\lambda=30$ - Safety};
%	\addplot [color=green,dashed,thick,mark=none,mark options={green,solid}]
%		table[x index=0,y index=1, col sep=comma]{figures/data/dataProbabilityGoalNoSafeLambda30.dat};
%	\addlegendentry{$\lambda=30$ - Goal};
%
%	\addplot [color=blue,solid,thick,mark=none,mark options={blue,solid}]
%		table[x index=0,y index=1, col sep=comma]{figures/data/dataProbabilitySafetyNoSafeLambda60.dat};
%	\addlegendentry{$\lambda=60$ - Safety};
%	\addplot [color=blue,dashed,thick,mark=none,mark options={blue,solid}]
%		table[x index=0,y index=1, col sep=comma]{figures/data/dataProbabilityGoalNoSafeLambda60.dat};
%	\addlegendentry{$\lambda=60$ - Goal};
%	
%\end{axis}
%\end{tikzpicture}

\begin{tikzpicture}
	\pgfplotsset{grid style={dashed,gray!50}}
	\begin{axis}[
		tick scale binop=\times,
		%title style={yshift=-1ex},
		%xlabel near ticks,
		%ylabel near ticks,
		minor tick num=1,
		%title={},
		xlabel={Iteration ($k$)},
		ylabel={Probability},
		ylabel near ticks,
		width=\columnwidth, 
		height=0.75\columnwidth, 
		xmin=0,xmax=10000,ymin=0,ymax=1,
		grid=both,
		legend entries={
			$\lambda=0$,
        	Safety Level,
         	$\lambda=30$,
         	Success Probability,
         	$\lambda=60$,
         	 \enskip},
		legend columns=2,
		legend style={
			at={(0.98,0.24)}, 
			anchor=south east, 
			legend cell align=left
			}
	]
	\addlegendimage{no markers, red,thick}
	\addlegendimage{no markers,black,solid,thick}
	\addlegendimage{no markers, green,thick}
	\addlegendimage{no markers,black,dashed,thick}
	\addlegendimage{no markers, blue,thick}	
	\addlegendimage{empty legend,thick}
	
	\addplot [color=red,solid,thick,mark=none,mark options={red,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataProbabilitySafetyNoSafeLambda0.dat};
	\addplot [color=red,dashed,thick,mark=none,mark options={red,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataProbabilityGoalNoSafeLambda0.dat};

	\addplot [color=green,solid,thick,mark=none,mark options={green,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataProbabilitySafetyNoSafeLambda30.dat};
	\addplot [color=green,dashed,thick,mark=none,mark options={green,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataProbabilityGoalNoSafeLambda30.dat};

	\addplot [color=blue,solid,thick,mark=none,mark options={blue,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataProbabilitySafetyNoSafeLambda60.dat};
	\addplot [color=blue,dashed,thick,mark=none,mark options={blue,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataProbabilityGoalNoSafeLambda60.dat};
	
\end{axis}
\end{tikzpicture}




==> fig_probabilities_Safe.tex <==
%!TEX root = root.tex
\begin{tikzpicture}
	\pgfplotsset{grid style={dashed,gray!50}}
	\begin{axis}[
		tick scale binop=\times,
		%title style={yshift=-1ex},
		%xlabel near ticks,
		%ylabel near ticks,
		minor y tick num=0,
		minor x tick num=1,
		ytick={0,0.2,0.4,...,1},
		%title={},
		xlabel={Iteration ($k$)},
		ylabel={Probability},
		ylabel near ticks,
		width=\columnwidth, 
		height=0.45\columnwidth, 
		xmin=0,xmax=10000,ymin=0,ymax=1,
		grid=both,
		legend style={
			at={(0.98,0.06)}, 
			anchor=south east, 
			legend cell align=left
			}
	]
	\addplot [color=red,solid,thick,mark=none,mark options={red,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataProbabilitySafetySafe.dat};
	\addlegendentry{Safety Level};
			
	\addplot [color=red,dashed,thick,mark=none,mark options={red,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataProbabilityGoalSafe.dat};
	\addlegendentry{Success Probability};
	
\end{axis}
\end{tikzpicture}

